Approximating the Shapley Value without Marginal Contributions

The Shapley value, which is arguably the most popular approach for assigning a meaningful contribution value to players in a cooperative game, has recently been used intensively in explainable artificial intelligence. Its meaningfulness is due to axiomatic properties that only the Shapley value satisfies, which, however, comes at the expense of an exact computation growing exponentially with the number of agents. Accordingly, a number of works are devoted to the efficient approximation of the Shapley value, most of them revolve around the notion of an agent's marginal contribution. In this paper, we propose with SVARM and Stratified SVARM two parameter-free and domain-independent approximation algorithms based on a representation of the Shapley value detached from the notion of marginal contribution. We prove unmatched theoretical guarantees regarding their approximation quality and provide empirical results including synthetic games as well as common explainability use cases comparing ourselves with state-of-the-art methods.

==> figures/stratified_svarm_figure.tex <==
\definecolor{urn}{HTML}{E6E6E6}

\begin{figure*}[ht]
\centering
\begin{tikzpicture}[scale = 0.8]
	\coordinate (c1) at (0,0);
	\coordinate (c2) at (5.8,0);
	\coordinate (c3) at (12,0);
	\coordinate (c4) at (17.5,0);
	\coordinate (r+) at (0,3.8);
	\coordinate (r-) at (0,0);
	\coordinate (gap) at (0.6,0);
	\coordinate (Gap) at (1.4,0);
	\coordinate (height) at (0,1.3);
	\coordinate (width) at (2,0);
	\coordinate (meanDown) at (0,0.4);
	\coordinate (Uup) at (0,0.4);
	\coordinate (Uright) at (0.25,0);
	\coordinate (boxHmargin) at (0.3,0);
	\coordinate (boxVmargin) at (0,0.2);
	\coordinate (boxDown) at (0,1.1);
	\coordinate (formulaUp) at (0,0.2);
	\coordinate (playerUp) at (0,0.45);
	\coordinate (playerLeft) at (0.3,0);
	\coordinate (sampleCorner) at ($(c4) - (boxDown) - (boxVmargin)$);
	\coordinate (sampleHeight) at ($2*(boxVmargin) + (boxDown) + (r+) + (height)$);
	\coordinate (sampleWidth) at (3.4,0);
	
	
	% Urns player 1 positive
	\draw[draw=urn, fill=urn] ($(c1) + (r+)$) rectangle ($(c1) + (r+) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c1) + (r+)$) -- ($(c1) + (height) + (r+)$);
	\draw[thick] ($(c1) + (width) + (r+)$) -- ($(c1) + (width) + (height) + (r+)$);
	\draw[thick] ($(c1) + (width) + (r+) + (gap)$) -- ($(c1) + (width) + (height) + (r+) + (gap)$);
	\draw[thick] ($(c1) + (width) + (r+) + 2*(gap)$) -- ($(c1) + (width) + (height) + (r+) + 2*(gap)$);
	\draw[thick] ($(c1) + (width) + (r+) + 2*(gap) + (Gap)$) -- ($(c1) + (width) + (height) + (r+) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c1) + (width) + (r+) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r+) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r+) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r+)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c1) + 0.5*(width) + (Uup) + (r+)$) {$U_{1,0}^+$};
	\node[scale=0.8] at ($(c1) + 0.5*(width) + (Uup) + (r+) + 2*(gap) + (Gap) + (Uright)$) {$U_{1,n-1}^+$};
	%\node[scale=0.65] at ($(c1) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_{1,0}^+$}};
	%\node[scale=0.65] at ($(c1) + 0.5*(width) + (r+) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{red}{$\phi_{1,n-1}^+$}};
    \node[scale=0.65] at ($(c1) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_{1,0}^+$}};
	\node[scale=0.65] at ($(c1) + 0.5*(width) + (r+) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{red}{$\phi_{1,n-1}^+$}};
	
	% Urns player 1 negative
	\draw[draw=urn, fill=urn] ($(c1) + (r-)$) rectangle ($(c1) + (r-) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c1) + (r-)$) -- ($(c1) + (height) + (r-)$);
	\draw[thick] ($(c1) + (width) + (r-)$) -- ($(c1) + (width) + (height) + (r-)$);
	\draw[thick] ($(c1) + (width) + (r-) + (gap)$) -- ($(c1) + (width) + (height) + (r-) + (gap)$);
	\draw[thick] ($(c1) + (width) + (r-) + 2*(gap)$) -- ($(c1) + (width) + (height) + (r-) + 2*(gap)$);
	\draw[thick] ($(c1) + (width) + (r-) + 2*(gap) + (Gap)$) -- ($(c1) + (width) + (height) + (r-) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c1) + (width) + (r-) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r-) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r-) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c1) + (width) + (r-)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c1) + 0.5*(width) + (Uup) + (r-)$) {$U_{1,0}^-$};
	\node[scale=0.8] at ($(c1) + 0.5*(width) + (Uup) + (r-) + 2*(gap) + (Gap) + (Uright)$) {$U_{1,n-1}^-$};
    \node[scale=0.65] at ($(c1) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_{1,0}^-$}};
	\node[scale=0.65] at ($(c1) + 0.5*(width) + (r-) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{blue}{$\phi_{1,n-1}^-$}};
	
	% Player 1 box and formula
	\draw[dashed] ($(c1) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c1) + (r+) + (width) + 2*(gap) + (Gap) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c1) + 0.5*(width) + (gap) + 0.5*(Gap) - (playerLeft) + (r+) + (height) + (boxHmargin) + (playerUp)$) {Player 1};
    \node[scale=0.75] at ($(c1) + 0.5*(width) + (gap) + 0.5*(Gap) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_1 = \frac1n \sum\limits_{\ell=0}^{n-1} \textcolor{red}{\phi_{1,\ell}^+} - \textcolor{blue}{\phi_{1,\ell}^-}$};
	
	% Urns player 2 positive
	\draw[draw=urn, fill=urn] ($(c2) + (r+)$) rectangle ($(c2) + (r+) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c2) + (r+)$) -- ($(c2) + (height) + (r+)$);
	\draw[thick] ($(c2) + (width) + (r+)$) -- ($(c2) + (width) + (height) + (r+)$);
	\draw[thick] ($(c2) + (width) + (r+) + (gap)$) -- ($(c2) + (width) + (height) + (r+) + (gap)$);
	\draw[thick] ($(c2) + (width) + (r+) + 2*(gap)$) -- ($(c2) + (width) + (height) + (r+) + 2*(gap)$);
	\draw[thick] ($(c2) + (width) + (r+) + 2*(gap) + (Gap)$) -- ($(c2) + (width) + (height) + (r+) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c2) + (width) + (r+) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r+) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r+) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r+)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c2) + 0.5*(width) + (Uup) + (r+)$) {$U_{2,0}^+$};
	\node[scale=0.8] at ($(c2) + 0.5*(width) + (Uup) + (r+) + 2*(gap) + (Gap) + (Uright)$) {$U_{2,n-1}^+$};
    \node[scale=0.65] at ($(c2) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_{2,0}^+$}};
	\node[scale=0.65] at ($(c2) + 0.5*(width) + (r+) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{red}{$\phi_{2,n-1}^+$}};
	
	% Urns player 2 negative
	\draw[draw=urn, fill=urn] ($(c2) + (r-)$) rectangle ($(c2) + (r-) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c2) + (r-)$) -- ($(c2) + (height) + (r-)$);
	\draw[thick] ($(c2) + (width) + (r-)$) -- ($(c2) + (width) + (height) + (r-)$);
	\draw[thick] ($(c2) + (width) + (r-) + (gap)$) -- ($(c2) + (width) + (height) + (r-) + (gap)$);
	\draw[thick] ($(c2) + (width) + (r-) + 2*(gap)$) -- ($(c2) + (width) + (height) + (r-) + 2*(gap)$);
	\draw[thick] ($(c2) + (width) + (r-) + 2*(gap) + (Gap)$) -- ($(c2) + (width) + (height) + (r-) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c2) + (width) + (r-) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r-) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r-) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c2) + (width) + (r-)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c2) + 0.5*(width) + (Uup) + (r-)$) {$U_{2,0}^-$};
	\node[scale=0.8] at ($(c2) + 0.5*(width) + (Uup) + (r-) + 2*(gap) + (Gap) + (Uright)$) {$U_{2,n-1}^-$};
    \node[scale=0.65] at ($(c2) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_{2,0}^-$}};
	\node[scale=0.65] at ($(c2) + 0.5*(width) + (r-) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{blue}{$\phi_{2,n-1}^-$}};
	
	% Player 2 box and formula
	\draw[dashed] ($(c2) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c2) + (r+) + (width) + 2*(gap) + (Gap) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c2) + 0.5*(width) + (gap) + 0.5*(Gap) - (playerLeft) + (r+) + (height) + (boxHmargin) + (playerUp)$) {Player 2};
    \node[scale=0.75] at ($(c2) + 0.5*(width) + (gap) + 0.5*(Gap) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_2 = \frac1n  \sum\limits_{\ell=0}^{n-1} \textcolor{red}{\phi_{2,\ell}^+} - \textcolor{blue}{\phi_{2,\ell}^-}$};
	
	\node[thick] at ($0.5*(c2) + 0.5*(c3) + 0.5*(width) + (gap) + 0.5*(Gap) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\cdots$};
	
	% Urns player n positive
	\draw[draw=urn, fill=urn] ($(c3) + (r+)$) rectangle ($(c3) + (r+) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c3) + (r+)$) -- ($(c3) + (height) + (r+)$);
	\draw[thick] ($(c3) + (width) + (r+)$) -- ($(c3) + (width) + (height) + (r+)$);
	\draw[thick] ($(c3) + (width) + (r+) + (gap)$) -- ($(c3) + (width) + (height) + (r+) + (gap)$);
	\draw[thick] ($(c3) + (width) + (r+) + 2*(gap)$) -- ($(c3) + (width) + (height) + (r+) + 2*(gap)$);
	\draw[thick] ($(c3) + (width) + (r+) + 2*(gap) + (Gap)$) -- ($(c3) + (width) + (height) + (r+) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c3) + (width) + (r+) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r+) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r+) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r+)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c3) + 0.5*(width) + (Uup) + (r+)$) {$U_{n,0}^+$};
	\node[scale=0.8] at ($(c3) + 0.5*(width) + (Uup) + (r+) + 2*(gap) + (Gap) + (Uright)$) {$U_{n,n-1}^+$};
    \node[scale=0.65] at ($(c3) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_{n,0}^+$}};
	\node[scale=0.65] at ($(c3) + 0.5*(width) + (r+) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{red}{$\phi_{n,n-1}^+$}};
	
	% Urns player n negative
	\draw[draw=urn, fill=urn] ($(c3) + (r-)$) rectangle ($(c3) + (r-) + (width) + 2*(gap) + (Gap) + (height)$);
	\draw[thick] ($(c3) + (r-)$) -- ($(c3) + (height) + (r-)$);
	\draw[thick] ($(c3) + (width) + (r-)$) -- ($(c3) + (width) + (height) + (r-)$);
	\draw[thick] ($(c3) + (width) + (r-) + (gap)$) -- ($(c3) + (width) + (height) + (r-) + (gap)$);
	\draw[thick] ($(c3) + (width) + (r-) + 2*(gap)$) -- ($(c3) + (width) + (height) + (r-) + 2*(gap)$);
	\draw[thick] ($(c3) + (width) + (r-) + 2*(gap) + (Gap)$) -- ($(c3) + (width) + (height) + (r-) + 2*(gap) + (Gap)$);
	\draw[thick, fill=urn] ($(c3) + (width) + (r-) + 2*(gap) + (Gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r-) + 2*(gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r-) + (gap)$) arc [radius=1.0, start angle=0, end angle=-180];
	\draw[thick, fill=urn] ($(c3) + (width) + (r-)$) arc [radius=1.0, start angle=0, end angle=-180];
	\node[scale=0.8] at ($(c3) + 0.5*(width) + (Uup) + (r-)$) {$U_{n,0}^-$};
	\node[scale=0.8] at ($(c3) + 0.5*(width) + (Uup) + (r-) + 2*(gap) + (Gap) + (Uright)$) {$U_{n,n-1}^-$};
    \node[scale=0.65] at ($(c3) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_{n,0}^-$}};
	\node[scale=0.65] at ($(c3) + 0.5*(width) + (r-) - (meanDown) + 2*(gap) + (Gap) + (Uright)$) {\textcolor{blue}{$\phi_{n,n-1}^-$}};
	
	% Player n box and formula
	\draw[dashed] ($(c3) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c3) + (r+) + (width) + 2*(gap) + (Gap) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c3) + 0.5*(width) + (gap) + 0.5*(Gap) - (playerLeft) + (r+) + (height) + (boxHmargin) + (playerUp)$) {Player $n$};
    \node[scale=0.75] at ($(c3) + 0.5*(width) + (gap) + 0.5*(Gap) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_n = \frac1n \sum\limits_{\ell=0}^{n-1} \textcolor{red}{\phi_{n,\ell}^+} - \textcolor{blue}{\phi_{n,\ell}^-}$};
	
	% Sampling
	\draw[thick, fill=urn, draw=black] (sampleCorner) rectangle ($(sampleCorner) + (sampleWidth) + (sampleHeight)$);
	\node[scale=0.7, align=left] at ($(sampleCorner) + 0.5*(sampleWidth) + 0.68*(sampleHeight)$) {$\bullet$ Sample $s \sim \tilde{P}$ \\ \\ $\bullet$ Sample $A$ uniformly \\ \hspace{0.25cm} with size $s$ \\ \\ $\bullet$ Update all $\hat\phi_{i,s-1}^+$ \\ \hspace{0.25cm} with $i \in A$ \\ \\ $\bullet$ Update all $\hat\phi_{i,s}^-$ \\ \hspace{0.25cm} with $i \notin A$};
	\node[scale=0.7, align=center] at ($(sampleCorner) + 0.5*(sampleWidth) + 0.28*(sampleHeight)$) {$s=3$, $A = \{1,3,5\}:$};
	\node[scale=0.7, align=left] at ($(sampleCorner) + 0.5*(sampleWidth) + 0.16*(sampleHeight)$) {$\rightarrow$ Update \textcolor{red}{$\hat\phi_{1,2}^+, \hat\phi_{3,2}^+, \hat\phi_{5,2}^+$} \\ $\rightarrow$ Update \textcolor{blue}{$\hat\phi_{2,3}^-, \hat\phi_{4,3}^-$}};
	\node[scale=0.7, align=center] at ($(c4) + (r+) + 0.5*(sampleWidth) + (height) + (playerUp)$) {$\mathcal{N}=\{1,2,3,4,5\}$};
\end{tikzpicture}
\vspace{-0.8em}
\vspace{0.1in}
\caption{Illustration of Stratified SVARM's update rule: Each player i has urns $U_{i,\ell}^+ := \{S \cup \{i\} \mid S \subseteq \mathcal{N}_i, |S|=\ell\}$ and \mbox{$U_{i,\ell}^- := \{S \mid S \subseteq \mathcal{N}_i, |S| = \ell \}$} for all $\ell \in \{0,\ldots,n-1\}$ containing marbles representing coalitions, with mean coalition worths $\phi_{i,\ell}^+$ and $\phi_{i,\ell}^-$.
Each sampled coalition is used to update the estimates of all players' urns that contain the corresponding marble.}
\label{fig:Stratified}
\end{figure*}

==> figures/svarm_figure.tex <==
\definecolor{urn}{HTML}{E6E6E6}

\begin{figure*}[ht]
\centering
\begin{tikzpicture}[scale = 0.8]
	\coordinate (c1) at (0,0);
	\coordinate (c2) at (3.9,0);
	\coordinate (c3) at (8.3,0);
	\coordinate (c4) at (12.2,0);
	\coordinate (r+) at (0,3.8);
	\coordinate (r-) at (0,0);
	\coordinate (height) at (0,1.3);
	\coordinate (width) at (2.4,0);
	\coordinate (boxHmargin) at (0.3,0);
	\coordinate (boxVmargin) at (0,0.2);
	\coordinate (boxDown) at (0,1.2);
	\coordinate (playerH) at (0.32,0);
	\coordinate (playerV) at (0,0.45);
	\coordinate (formulaW) at (1.1,0);
	\coordinate (formulaH) at (0,0.4);
	\coordinate (formulaUp) at (0,0.1);
	\coordinate (Uup) at (0,0.4);
	\coordinate (meanDown) at (0,0.5);
	\coordinate (frameHmargin) at (0.5,0);
	\coordinate (frameVmargin) at (0,0.6);
	\coordinate (sampleWidth) at (4.4,0);
	\coordinate (sampleHeight) at (0,2.7);
	\coordinate (PositiveCorner) at ($(c4) + (r+) - (0,1.2)$);
	\coordinate (NegativeCorner) at ($(c4) + (r-) - (boxVmargin) - (0,1.2)$);
	
	%\draw[thick] ($(c1) + (r-) - (boxDown) - (boxVmargin) - (boxHmargin) - (frameVmargin) - (frameHmargin)$) rectangle ($(c4) + (r+) + (sampleWidth) + (height) + (boxVmargin) + (frameVmargin) + (frameHmargin)$);
	
	% Urn player 1 positive
	\draw[draw=urn, fill=urn] ($(c1) + (r+)$) rectangle ($(c1) + (r+) + (width) + (height)$);
	\draw[thick] ($(c1) + (r+)$) -- ($(c1) + (height) + (r+)$);
	\draw[thick] ($(c1) + (width) + (r+)$) -- ($(c1) + (width) + (height) + (r+)$);
	\draw[thick, fill=urn] ($(c1) + (width) + (r+)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c1) + 0.5*(width) + (Uup) + (r+)$) {$U_1^+$};
	\node[scale=0.7] at ($(c1) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_1^+$}};
	
	% Urn player 1 negative
	\draw[draw=urn, fill=urn] ($(c1) + (r-)$) rectangle ($(c1) + (r-) + (width) + (height)$);
	\draw[thick] ($(c1) + (r-)$) -- ($(c1) + (height) + (r-)$);
	\draw[thick] ($(c1) + (width) + (r-)$) -- ($(c1) + (width) + (height) + (r-)$);
	\draw[thick, fill=urn] ($(c1) + (width) + (r-)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c1) + 0.5*(width) + (Uup) + (r-)$) {$U_1^-$};
	\node[scale=0.7] at ($(c1) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_1^-$}};
	
	% Player 1 box and formula
	\draw[dashed] ($(c1) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c1) + (r+) + (width) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c1) + 0.5*(width) - (playerH) + (r+) + (height) + (boxHmargin) + (playerV)$) {Player 1};
	\node[scale=0.8] at ($(c1) + 0.5*(width) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_1 = \textcolor{red}{\phi_1^+} - \textcolor{blue}{\phi_1^-}$};
	
	% Urn player 2 positive
	\draw[draw=urn, fill=urn] ($(c2) + (r+)$) rectangle ($(c2) + (r+) + (width) + (height)$);
	\draw[thick] ($(c2) + (r+)$) -- ($(c2) + (height) + (r+)$);
	\draw[thick] ($(c2) + (width) + (r+)$) -- ($(c2) + (width) + (height) + (r+)$);
	\draw[thick, fill=urn] ($(c2) + (width) + (r+)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c2) + 0.5*(width) + (Uup) + (r+)$) {$U_2^+$};
	\node[scale=0.7] at ($(c2) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_2^+$}};
	
	% Urn player 2 negative
	\draw[draw=urn, fill=urn] ($(c2) + (r-)$) rectangle ($(c2) + (r-) + (width) + (height)$);
	\draw[thick] ($(c2) + (r-)$) -- ($(c2) + (height) + (r-)$);
	\draw[thick] ($(c2) + (width) + (r-)$) -- ($(c2) + (width) + (height) + (r-)$);
	\draw[thick, fill=urn] ($(c2) + (width) + (r-)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c2) + 0.5*(width) + (Uup) + (r-)$) {$U_2^-$};
	\node[scale=0.7] at ($(c2) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_2^-$}};
	
	% Player 2 box and formula
	\draw[dashed] ($(c2) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c2) + (r+) + (width) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c2) + 0.5*(width) - (playerH) + (r+) + (height) + (boxHmargin) + (playerV)$) {Player 2};
	\node[scale=0.8] at ($(c2) + 0.5*(width) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_2 = \textcolor{red}{\phi_2^+} - \textcolor{blue}{\phi_2^-}$};

	\node[thick] at ($0.5*(c2) + 0.5*(c3) + 0.5*(width) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\cdots$};
	
	% Urn player n positive
	\draw[draw=urn, fill=urn] ($(c3) + (r+)$) rectangle ($(c3) + (r+) + (width) + (height)$);
	\draw[thick] ($(c3) + (r+)$) -- ($(c3) + (height) + (r+)$);
	\draw[thick] ($(c3) + (width) + (r+)$) -- ($(c3) + (width) + (height) + (r+)$);
	\draw[thick, fill=urn] ($(c3) + (width) + (r+)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c3) + 0.5*(width) + (Uup) + (r+)$) {$U_n^+$};
	\node[scale=0.7] at ($(c3) + 0.5*(width) + (r+) - (meanDown)$) {mean: \textcolor{red}{$\phi_n^+$}};
	
	% Urn player n negative
	\draw[draw=urn, fill=urn] ($(c3) + (r-)$) rectangle ($(c3) + (r-) + (width) + (height)$);
	\draw[thick] ($(c3) + (r-)$) -- ($(c3) + (height) + (r-)$);
	\draw[thick] ($(c3) + (width) + (r-)$) -- ($(c3) + (width) + (height) + (r-)$);
	\draw[thick, fill=urn] ($(c3) + (width) + (r-)$) arc [radius=1.2, start angle=0, end angle=-180];
	\node[scale=0.9] at ($(c3) + 0.5*(width) + (Uup) + (r-)$) {$U_n^-$};
	\node[scale=0.7] at ($(c3) + 0.5*(width) + (r-) - (meanDown)$) {mean: \textcolor{blue}{$\phi_n^-$}};
	
	% Player n box and formula
	\draw[dashed] ($(c3) + (r-) - (boxHmargin) - (boxDown) - (boxVmargin)$) rectangle ($(c3) + (r+) + (width) + (height) + (boxHmargin) + (boxVmargin)$);
	\node[scale=0.7] at ($(c3) + 0.5*(width) - (playerH) + (r+) + (height) + (boxHmargin) + (playerV)$) {Player $n$};
	\node[scale=0.8] at ($(c3) + 0.5*(width) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {$\phi_n = \textcolor{red}{\phi_n^+} - \textcolor{blue}{\phi_n^-}$};
	
	% Positive sampling
	\draw[thick, fill=urn, draw=black] (PositiveCorner) rectangle ($(PositiveCorner) + (sampleWidth) + (sampleHeight)$);
	\node[scale=0.7, align=left] at ($(PositiveCorner) + 0.5*(sampleWidth) + 0.7*(sampleHeight)$) {$\bullet$ Sample $A^+ \sim P^+$ \\ \\ $\bullet$ Update all $\hat\phi_i^+$ with $i \in A^+$};
	%\node[scale=0.7, align=center] at ($(PositiveCorner) + + 0.5*(sampleWidth) + 0.6*(sampleHeight)$) {$\bullet$ Update all $\hat\phi_i^+$ with $i \in A^+$};
	\node[scale=0.7, align=center] at ($(PositiveCorner) + + 0.5*(sampleWidth) + 0.25*(sampleHeight)$) {$A^+=\{1,3,5\} \in U_1^+, U_3^+, U_5^+$ \\ $\rightarrow$ Update \textcolor{red}{$\hat\phi_1^+, \hat\phi_3^+, \hat\phi_5^+$}};
	
	% Negative sampling
	\draw[thick, fill=urn, draw=black] (NegativeCorner) rectangle ($(NegativeCorner) + (sampleWidth) + (sampleHeight)$);
	\node[scale=0.7, align=left] at ($(NegativeCorner) + + 0.5*(sampleWidth) + 0.7*(sampleHeight)$) {$\bullet$ Sample $A^- \sim P^-$ \\ \\ $\bullet$ Update all $\hat\phi_i^-$ with $i \notin A^-$};
	%\node[scale=0.7, align=center] at ($(NegativeCorner) + + 0.5*(sampleWidth) + 0.6*(sampleHeight)$) {Update all $\hat\phi_i^-$ with $i \notin A^-$};
	\node[scale=0.7, align=center] at ($(NegativeCorner) + + 0.5*(sampleWidth) + 0.25*(sampleHeight)$) {$A^-=\{1,3,5\} \in U_2^-, U_4^-$ \\ $\rightarrow$ Update \textcolor{blue}{$\hat\phi_2^-, \hat\phi_4^-$}};
	
	\node[thick, scale=0.7] at ($(c4) + 0.5*(sampleWidth) + 0.5*(r+) + 0.5*(r-) + (formulaUp)$) {Alternate};
	\draw[-{latex}] ($(c4) + 0.5*(sampleWidth) + 0.5*(r+) + 0.5*(r-) + (formulaUp) + (0,0.15)$) -- ($(c4) + 0.5*(sampleWidth) + 0.5*(r+) + 0.5*(r-) + (formulaUp) + (0,0.55)$);
	\draw[-{latex}] ($(c4) + 0.5*(sampleWidth) + 0.5*(r+) + 0.5*(r-) + (formulaUp) - (0,0.2)$) -- ($(c4) + 0.5*(sampleWidth) + 0.5*(r+) + 0.5*(r-) + (formulaUp) - (0,0.65)$);
	\node[thick, scale=0.7] at ($(c4) + 0.5*(sampleWidth) + (r+) + (height) + (playerV)$) {$\mathcal{N} = \{1,2,3,4,5\}$};
	
\end{tikzpicture}
\vspace{-0.8em}
\vspace{0.1in}
\caption{Illustration of SVARM's sampling process and update rule: Each player $i$ has two urns $U_i^+ := \{S \cup \{i\} \mid S \subseteq \mathcal{N}_i\}$ and $U_i^- := \{S \mid S \subseteq \mathcal{N}_i\}$ containing marbles representing coalitions, with mean coalition worths $\phi_i^+$ and $\phi_i^-$.
SVARM alternates between sampling $A^+ \sim P^+$ and $A^- \sim P^-$.
With each drawn coalition all estimates of urns are updated which contain the corresponding marble.}
\label{fig:SVARM}
\end{figure*}
